Probabilistic 3d regression with projected huber distribution

Estimating probability distributions which describe where an object is likely to be from camera data is a task with many applications. In this work we describe properties which we argue such methods should conform to. We also design a method which conform to these properties. In our experiments we show that our method produces uncertainties which correlate well with empirical errors. We also show that the mode of the predicted distribution outperform our regression baselines. The code for our implementation is available online.

==> supp_constraint_2.tex <==
TODO

==> supp_moments.tex <==
\label{sec:supp_moments}
Here we derive the moments up to the second moment.

\begin{align}
E\begin{bmatrix}
x/z \\ y/z
\end{bmatrix} &= \mu_p\\
Var\begin{bmatrix}
x/z \\ y/z
\end{bmatrix} &\propto A^{-1}A^{-1} \dfrac {(\Gamma(-2/a,1) + \Gamma(2/a,1))} {2\Gamma(0,1)} \\
E\left[z \right] &= \dfrac {\Gamma(1/a,1) + \Gamma(-1/a,1)} {2\Gamma(0,1)} \mu_z\\
Var\left[z \right] &= \dfrac {2\Gamma(0,1)(\Gamma(2/a,1) + \Gamma(-2/a,1)) - (\Gamma(1/a,1)+\Gamma(-1/a,1))^2} {4\Gamma(0,1)^2} \mu_z^2\\
E\left[log(z) \right] &= \mu_z \\
Var\left[log(z) \right] &\propto 1/a^2
\end{align}

In practice, for the allowed values for $a$ the Gamma fraction range between $1$ to $1.28$ for the expression determining $Var[x/z, y/z]$.
The expected value of $z$ is $\mu_z$ adjusted by an expression of a. The gamma term for $E[z]$ range between 1.07 and 1.0, for the allowed range of $a$. \textit{the analytical formula of the variance is quite hard to parse.}

\textbf{Proof of projected coordinates}

For this proof we will use the notation
\begin{equation}
v_p = \begin{bmatrix}
x/z \\ y/z
\end{bmatrix}
\end{equation}
This is slightly different than the notation in the rest of the work


\begin{align}
E\begin{bmatrix}
x/z \\ y/z
\end{bmatrix} &= \dfrac{1} {K(A, \mu, a)}
    \int \begin{bmatrix}
x/z \\ y/z
\end{bmatrix} \exp\left(-h\left(\left\|A\begin{bmatrix} x/z-\mu_x \\ y/z-\mu_y \end{bmatrix}\right\|_2\dfrac{z}{\mu_z}\right)
    - \log(z/\mu_z) - \exp(a|\log(z/\mu_z)|)\right) dxdydz \\
&= \mu_p + \dfrac {1} {(2\Gamma(0,1))(1+\exp(-1/2))} \int\limits_{-\infty}^{\infty} \exp(-s/a) A^{-1}\int\limits_{\mathbb{R}^2} q \exp(-h(\|q\|_2))dq\exp(-\exp(|s|))ds \\
&= \mu_p
\end{align} 

The first step is doing the same basis change as equation \ref{eq:basis_change_norm_factor_1} and \ref{eq:basis_change_norm_factor_2} with
\begin{equation}
v_p = \mu_p + A^{-1}q\dfrac{z} {\mu_z}
\end{equation}

Since $\mu_p$ is does not depend on the variables we integrate over we know the expected value of it is itself.

The second step is realizing that the distribution is symmetric with respect to $q$. Therefore the expected value of $q$ is 0.

We now compute 
\begin{align}
    Var\left[v_p\right] &= E\left[v_p v_p^T\right] - E\left[v_p\right] E\left[v_p^T\right] \\
    &= E\left[\mu_p \mu_p^T + \mu_p q^TA^{-1}z\mu_z + A^{-1}q\mu_z^Tz\mu_z + A^{-1}qq^TA^{-1}\dfrac{z^2}{\mu_z^2}\right] - \mu_p \mu_p^T \\
    &= E\left[A^{-1}qq^TA^{-1}\exp(2s/a)\right] \\ 
    &= A^{-1}E\left[qq^T\exp(2s/a)\right]A^{-1}
\end{align}

\begin{align}
    E\left[qq^T\exp(2s/a)\right]
    &= \dfrac {1}{K(A,\mu,a)} \int\limits_{0}^{\infty} \int\limits_{\mathbb{R}^2} qq^T\exp(-h(\|q\|))dq \exp(2s/a) \exp(-\exp(|s|))ds \\
    &= \dfrac {I} {2\pi(2\Gamma(0,1))(1+\exp(-1/2))}
    \int\limits_{0}^{\infty}\int\limits_{0}^{2\pi} r^3\cos^2(\theta) \exp(-h(r)) d\theta dr \\
    & (\int\limits_{0}^{\infty} \exp(-2s/a -\exp(s))ds + \int\limits_{0}^{\infty} \exp(2s/a -\exp(s))ds) \\
    &= I \dfrac {\pi(13\exp(-1/2)+2)(\Gamma(-2/a, 1) + \Gamma(2/a, 1))} {2\pi(2\Gamma(0,1))(1+\exp(-1/2))} \\
    &= I \dfrac {(13\exp(-1/2)+2)(\Gamma(-2/a, 1) + \Gamma(2/a, 1))} {2(2\Gamma(0,1))(1+\exp(-1/2))}
\end{align}

Putting this together with the computation for the variance concludes the proof.

\textbf{proof of expected z coordinate}

First note $z = \exp(s/a)\mu_z$
\begin{align}
E\left[z\right] &= \dfrac {\int\limits_{\infty}^{\infty} \exp(s/a-\exp(|s|))\mu_z} {\int\limits_{\infty}^{\infty} \exp(\exp(|s|))} \\
&= \dfrac {\Gamma(1/a,1)+\Gamma(-1/a,1)} {2\Gamma(0,1)}\mu_z
\end{align}

\begin{align}
E\left[z^2\right] &= \dfrac {\int\limits_{\infty}^{\infty} \exp(2s/a-\exp(|s|))\mu_z^2} {\int\limits_{\infty}^{\infty} \exp(\exp(|s|))} \\
&= \dfrac {\Gamma(2/a,1)+\Gamma(-2/a,1)} {2\Gamma(0,1)}\mu_z^2
\end{align}
Which gives


==> supp_proof_basis_change.tex <==
In this section we prove that the negative log likelihood of 
equation \ref{eq:norm_factor_prob} result in equation \ref{eq:loss_after_basis_change} after the parameter change in \ref{eqs:basis_change_variables} and \ref{eqs:basis_change_parameters}

We state these equations for reference

\begin{equation}
    p(x,y,z) = \dfrac{1} {K(A, \mu, a)} \exp(-h\left(\left\|A\begin{bmatrix} x/z-\mu_x \\ y/z-\mu_y \end{bmatrix}\right\|_2\dfrac{z}{\mu_z}\right) - \log(z/\mu_z) - \exp(h(a|\log(z/\mu_z)|)))
\end{equation}

\begin{align}
    v_p = \begin{bmatrix} x_p \\ y_p \end{bmatrix} &= \begin{bmatrix} \dfrac{2fx} {zS} \\ \dfrac{2fy} {zS} \end{bmatrix} \\  
    z_p &= \log\left(\dfrac{zS} {\mu_{z0}f}\right) / D \\ 
    b &= a*D \\
    \nu_v = \begin{bmatrix} \nu_x \\ \nu_y \end{bmatrix} &= \dfrac {f\mu_{z0}} {S\mu_z} A \begin{bmatrix} \mu_x \\ \mu_y \end{bmatrix} \\
    \nu_z &= a\log\left(\dfrac {\mu_zS} {\mu_{z0}f}\right) \\
    B &= \dfrac {A\mu_{z0}} {2\mu_z} 
\end{align}

The negative log likelihood with the original parameterization turns into

\begin{align}
\label{eq:loss_orig_basis_term_1}
    L(x,y,z;A,a,\mu) &= h\left(\left\|A\begin{bmatrix} x/z-\mu_x \\ y/z-\mu_y \end{bmatrix}\right\|_2\dfrac{z}{\mu_z}\right) \\
    \label{eq:loss_orig_basis_term_2}
    &+ \exp(h(a|\log(z/\mu_z)|)) \\
    \label{eq:loss_orig_basis_term_log_z_mu}
    &+ \log(z/\mu_z) \\
    &+ \log(K(A, \mu, a))
\end{align}

The term \ref{eq:loss_orig_basis_term_1} becomes

\begin{align}
&h\left(\left\|A\begin{bmatrix} x/z-\mu_x \\ y/z-\mu_y \end{bmatrix}\right\|_2\dfrac {z}{\mu_z}\right) = \\
&= h\left(\left\|A\begin{bmatrix} x/z \\ y/z \end{bmatrix}\ \dfrac{z} {\mu_z}- A\begin{bmatrix} \mu_x \\ \mu_y \end{bmatrix} \dfrac{z} {\mu_z} \right\|_2\right) = \\
&= h\left(\left\|\dfrac {2B\mu_z} {\mu_{z,0}} \dfrac{S}{2f}\begin{bmatrix} x_p \\ y_p \end{bmatrix} \dfrac{\exp(z_pD)f\mu_{z,0}} {S\mu_z} - \dfrac{\nu_v S \mu_z} {f \mu_{z,0}} \dfrac {f\mu_{z,0}} {S\mu_z} \exp(z_pD) \right\|_2\right) = \\
&= h\left(\left\|Bv_p-\nu_v\right\|_2\exp(z_pD)\right)
\end{align}

The term \ref{eq:loss_orig_basis_term_2} becomes

\begin{align}
\exp(h(a\log(z/\mu_z))) &= \exp(h\left(a \log\left(\dfrac{\exp^{z_pD} \dfrac {\mu_{z,0}f} {S}} {\exp^{\nu_z/a} \dfrac {\mu_{z,0}f} {S}}\right) \right)) \\
&= \exp(h(a(z_pD-\nu_z/a))) \\
&= \exp(h(bz_p-\nu_z))
\end{align}

From section \ref{sec:deriving_normalizing_factor} we know that the normalizing factor is 


\begin{equation}
K(A, \mu, a) = \dfrac {\mu_z^3} {|A|a}C_{norm\_constant}   
\end{equation}

therefore
\begin{align}
\label{eq:NLL_norm_factor}
\log(K(A, \mu, a)) &= 3\log(\mu_z) - \log(|A|) - \log(a) + \log(C_{norm\_constant}) \\
&= \log(\mu_z) - \log(|A\mu_{z0}/2\mu_z|) + 2\log(\mu_{z0}) - 2\log(2) - \log(aD) + \log(D) + log(C_{norm\_constant}) \\
&= \log(\mu_z) - \log(|B|) + 2\log(\mu_{z0}) - 2\log(2) - \log(b) + \log(D) + log(C_{norm\_constant})
\end{align}

We notice how the $\log(\mu_z)$ term will turn the term $\log(z/\mu_z)$ in equation \ref{eq:loss_orig_basis_term_log_z_mu} into $log(z)$.

here $log(C_{norm\_constant}$ swallows terms related to $S, f, \mu_{z,0},D$. The term $\log(\mu_z)$ will cancel out $\mu_z$ in $\log(z/\mu_z)$

In addition the variable change from $x,y,z$ to $x_p, y_p, z_p$ introduces a scale change corresponding to
\begin{align}
dv_p &= \dfrac{dv} {\begin{vmatrix}
  \dfrac{\partial x} {\partial x_p} & \dfrac{\partial x} {\partial y_p} & \dfrac{\partial x} {\partial z_p} \\
  \dfrac{\partial y} {\partial x_p} & \dfrac{\partial y} {\partial y_p} & \dfrac{\partial y} {\partial z_p} \\
  \dfrac{\partial z} {\partial x_p} & \dfrac{\partial z} {\partial y_p} & \dfrac{\partial z} {\partial z_p}
  \end{vmatrix}} \\
  &= \dfrac{dv} {\begin{vmatrix}
  2f/zS & 0 & -2fx/z^2S \\
  0 & 2f/zS & -2fy/z^2S \\
  0 & 0 & Dz \\
  \end{vmatrix}} \\
  &= \dfrac{ S^2zD} {4f^2}dv
\end{align}

This factor will result in the term
\begin{align}
   -\log{\dfrac{ S^2zD} {4f^2}} &= - \log(z) - \log{\dfrac{D S^2} {4f^2}}
\end{align}
in the loss. The $-log(z)$ term will cancel out $log(z)$ part of $log(z/\mu_z)$ in equation \ref{eq:loss_orig_basis_term_log_z_mu}, Since the $\mu_z$ part of the term was already canceled out by $\log(K(B, \nu, b))$ the $log(z/\mu_z)$ term is now completely canceled out. The other terms are constants for each sample and will not contribute to the gradients when training. Thus we can consider them part of $C_{norm\_constant}$ when analyzing the loss.

Adding the terms together yields equation \ref{eq:loss_after_basis_change}, concluding the proof.
